Digital Annealer for quadratic unconstrained binary optimization: a comparative performance analysis

Digital Annealer (DA) is a computer architecture designed for tackling combinatorial optimization problems formulated as quadratic unconstrained binary optimization (QUBO) models. In this paper, we present the results of an extensive computational study to evaluate the performance of DA in a systematic way in comparison to multiple state-of-the-art solvers for different problem classes. We examine pure QUBO models, as well as QUBO reformulations of three constrained problems, namely quadratic assignment, quadratic cycle partition, and selective graph coloring, with the last two being new applications for DA. For the selective graph coloring problem, we also present a size reduction heuristic that significantly increases the number of eligible instances for DA. Our experimental results show that despite being in its development stage, DA can provide high-quality solutions quickly and in that regard rivals the state of the art, particularly for large instances. Moreover, as opposed to established solvers, within its limit on the number of decision variables, DA's solution times are not affected by the increase in instance size. These findings illustrate that DA has the potential to become a successful technology in tackling combinatorial optimization problems.

==> PerformanceAnalysis_withGap.tex <==
\section{Performance Analysis}\label{performance_analysis}

In this section, we provide the results of our extensive experimental study which is conducted for comparing the performance of DA \cite{matsu2017} and three state-of-the-art solvers, namely GUROBI \cite{optimization2018}, CPLEX \cite{cplex2009v12}, and SCIP \cite{Achterberg2009}, on different problem classes and their benchmark instances from the literature or newly generated ones. %This kind of computational study does not exist in the literature to the best of our knowledge. 
Since DA inherently uses a heuristic (rather than an exact) algorithm, comparing the solutions produced by DA to those of solvers, which can yield provably optimal solutions, is an integral part of this study to gain insights into how close to optimal DA's solutions are. As such, we use different comparison measures which illustrate the results of each section in the best way. 

In what follows, we first focus on pure QUBO problems, and then %and analyze the performance of DA as well as commercial solvers on several well-known library instances. Then, we 
extend our study to constrained cases and consider quadratic assignment, quadratic cycle partition, and selective graph coloring problems.
%QAP and our Sel-Col application. 
%Note that we omit the results of SCIP for the latter case due to its inferiority to the other exact solvers. %as a new application area for DA and report the output of DA and the solvers for this specific problem. Finally, we introduce a new application of DA on graph coloring. More specifically, we describe Sel-Col and report the performance analysis accordingly.

\textcolor{red}{to Oylum: Please add experimental setup of DA and the other solvers, machine properties, etc. Also, need to mention the penalty coefficients.}

For DA experiments, we used the Digital Annealer environment prepared exclusively for research at the University of Toronto.
For experiments with GUROBI, CPLEX and SCIP, we used a Mac computer with 3 GHz Intel Core i5 CPU and 16 GB memory.
We use latest releases of all the solvers. In particular, we use the second generation of DA, GUROBI 9.0.3, CPLEX 12.10, and SCIP 7.0.1. 

%\nt{DA2; Gurobi 9.0.3; CPLEX 12.10}
% If the paper gets rejected, we can consider (i) Sensitivity analyses on the penalty coefficient, (ii) DA1 vs DA2 comparison, (iii) More problem classes, e.g., some from the DA literature


\os{AN OVERVIEW OF THE REST OF THIS SECTION WOULD HELP, CAN'T SEE THE BIG PICTURE NOW...}

%\os{IMHO, WE SHOULD GIVE A SUMMARY TABLE BEFORE WE DO THE DETAILED ANALYSIS. IT IS HARD TO INFER TAKEAWAY MESSAGES FROM THE SCATTERED DISCUSSION THAT FOLLOWS...}


\subsection{QUBO Benchmarks}

Our first set of experiments concerns pure QUBO problems; the problems that are originally modeled as QUBO, in other words, {\cred as a model \eqref{QUBO_model} with $P=1$}. We collect pure QUBO instances of varying sizes from well-known libraries; namely, OR-Library\footnote{
\href{http://people.brunel.ac.uk/~mastjjb/jeb/orlib/bqpinfo.html}{http://people.brunel.ac.uk/~mastjjb/jeb/orlib/bqpinfo.html}
} \cite{beasley1990or}, Biq-Mac\footnote{
\href{http://biqmac.uni-klu.ac.at/biqmaclib.html}{http://biqmac.uni-klu.ac.at/biqmaclib.html}
} \cite{wiegele2007biq}, and QPLIB\footnote{
\href{http://qplib.zib.de}{http://qplib.zib.de}
} \cite{furini2018qplib}. From OR-Library, we use test instances in \cite{beasley1998heuristic}, which have 20 to 2500 variables. Biq-Mac is a library that contains medium-size QUBO problem instances with 20 to 500 variables, some of them being the same as those offered by OR-library. Finally, QPLIB is a comprehensive library for quadratic programming that involves 23 pure QUBO problems with 120 to 1225 variables. Using these three libraries, we obtain 208 pure QUBO instances in total which contain 20 to 2500 variables. All of these instances are eligible for DA. Pure QUBO test set  information is summarized in 
Table \ref{tab:pureQUBO_instance_info}. %contains the number instances collected from each library along with the range of the number of variables in them.

\input{tables/pureQUBO_instance_info}

We note that for 3 of the 23 instances from QPLIB, instance parameters are beyond the acceptable ranges for DA.
%we encountered overflow errors (i.e., numerical issues) in parallel mode DA because of the large coefficients in the problem. 
Therefore, we present the experimental results for the remaining 205 instances in total. 

In order to evaluate the performance of DA and the solvers, in this section, we use the optimality gap as a measure of comparison, which is defined as 
$$\% \ \text{gap} = \frac{\text{UB}-\text{LB}}{|\text{UB}|}\cdot 100$$ 
where UB and LB denote (for a minimization problem) the upper bound and lower bound on the optimal value, respectively. However, since DA only yields feasible solutions, i.e., upper bounds, we use the best lower bound found by the exact solvers as the LB value in computing the gap value for every method. To make a fair comparison, we also use the best lower bound values when calculating the gap values of the solvers, instead of their own lower bounds.

%The pair of columns under the ``Total" heading in Table \ref{tab:pureQUBO_instance_info} provides the total number of instances and the limits on the number of variables, before they have been filtered out for eligibility for DA. The last pair of columns under the ``Eligible for DA" shows the same set of information for the instances that remain after discarding the ones that have a larger size than DA can manage.


%For our computational experiments, we explored some candidate solvers than can handle QUBO problems. We use CPLEX and GUROBI both to solve constrained {\it integer programming} (IP) problems under consideration, and their QUBO formulations. Beside these solvers, we also utilize the well-known nonlinear programming solver SCIP in our experimental study. 

\subsubsection{Exact solver comparison}

%\nt{The computational study is conducted on all of the instances collected from the three libraries mentioned before.}
%As the next step, we broaden our experimental set by including all of the instances collected from the three libraries mentioned before. Normally, this makes a total of 195 pure QUBO instances with 20 to 1000 variables. However, for 3 out of the 20 eligible instances from QPLIB, we encounter overflow errors in DA. Therefore, we present the experimental results for the remaining 192 instances. 

We begin with the comparison of the three exact solvers. 
% \begin{figure}[ht]
%     \centering
% 	\begin{subfigure}{0.49\textwidth}
% 		\centering
% 	    \includegraphics[scale=0.62]{figures/pyFig/pureQUBO/qubo_gap_cgs_10min.pdf}
% 		\caption{Over the full test set \nt{Analysis on full set of data}}
% 		\label{subfig:pureQUBO_gap_exact_solvers}
% 	\end{subfigure}
% 	\begin{subfigure}{0.49\textwidth}
% 		\centering
%         \includegraphics[scale=0.62]{figures/pyFig/pureQUBO/qubo_gap_cgs_10min_zoom_upto145.pdf}
%         \caption{Over the subset of the instances in the flatter part of (a) \nt{Magnifying the results for subset of part (a) data}}
%         \label{subfig:pureQUBO_gap_exact_solvers_zoomed}
% 	\end{subfigure}
% 	\begin{subfigure}{0.49\textwidth}
% 		\centering
%         \includegraphics[scale=0.62]{figures/pyFig/pureQUBO/qubo_gap_gs_10min_zoom_upto75.pdf}
%       \caption{Over the subset of the instances in the flatter part of (b) \nt{Further magnification of the results for subset of part (b) data}}
%         \label{subfig:pureQUBO_gap_exact_solvers_zoomed2}
% 	\end{subfigure}
% 	\caption{Performance comparison of exact solvers \nt{with 10-minute time limit} for pure QUBO instances}
% 	\label{fig:pureQUBO_exact_solvers}
% \end{figure}
\begin{figure}[ht]
    \centering
	\includegraphics[scale=0.72]{figures/newPureQUBO/ExactSolvers_10min_modified.pdf}
	\caption{Performance comparison of exact solvers with 10-minute time limit for pure QUBO instances}
	\label{fig:pureQUBO_exact_solvers}
\end{figure}
Figure \ref{fig:pureQUBO_exact_solvers} displays a comparison of the performances of the three solvers, where the runs are taken with a 10-minute time limit for each solver. The $x$-axis corresponds to the instances which are sorted based on the number of decision variables, while the $y$-axis shows the \% gap values. The instances that the solvers provide \% gap values larger than 100\% for them are illustrated on the upper part of the figures with appropriate markers. The figure includes the results of all instances in our QUBO test set, and signifies that CPLEX and SCIP are  outperformed by GUROBI specially in large instances. Additionally, it can be observed that SCIP provides huge \% gaps for most of the instances. 
%As the difference of the results are not easily distinguishable in the flat part of Figure \ref{subfig:pureQUBO_gap_exact_solvers}, we zoom into that part in Figure \ref{subfig:pureQUBO_gap_exact_solvers_zoomed}. There we observe that CPLEX still seems to be outperformed by GUROBI. After further magnifying the relatively flat parts of the plot in Figure \ref{subfig:pureQUBO_gap_exact_solvers_zoomed2}, we conclude that GUROBI is the best performing solver among the three. 

\subsubsection{DA mode comparison}
Next, we evaluate the performances of normal and parallel modes of DA. When running in normal mode, we use the best parameter combination we found after some preliminary testing, albeit not so thoroughly. As illustrated in Figure \ref{fig:pureQUBO_da_vs_da}, we find that, in general, the two modes of DA yield almost the same level of performance where the average running time of normal mode (0.4 seconds) is significantly less than that of parallel mode (67.36 seconds). It is also noticeable from the figure that the normal mode outperforms the parallel one in some larger instances.

% \begin{figure}[ht]
%     \centering
% 	\includegraphics[scale=0.62]{figures/pyFig/pureQUBO/qubo_gap_da_vs_da.pdf}
% 	\caption{Performance comparison of modes of DA for pure QUBO instances}
% 	\label{fig:pureQUBO_da_vs_da}
% \end{figure}
 
\begin{figure}[ht]
    \centering
	\includegraphics[scale=0.72]{figures/newPureQUBO/DA_ParallelNormal_60s.pdf}
	\caption{Performance comparison of modes of DA for pure QUBO instances}
	\label{fig:pureQUBO_da_vs_da}
\end{figure}

\subsubsection{Effect of variable ordering for DA}
%variable ordering
In order to have a better inside into the performance of DA, we also analyze the effect of input format on the output of DA; namely, the impact of different variable orderings; inspired by the fact the variable ordering can make a big difference in solution times for mixed-integer linear programs. For this purpose, we take a sample of five pure QUBO problem instances with 1000 variables, and experiment with 100 different random permutations for variable indices both in normal and parallel modes of DA. For normal mode, we try two different parameter combinations; an arbitrarily selected one that is not specifically tuned, and the one obtained as the best combination after our tuning efforts. 

\input{tables/pureQUBO_var_ordering}


Table \ref{tab:pureQUBO_var_ordering} summarizes the results of our tests with different variable orderings. For each one of the three alternative configurations, namely the parallel mode, the normal mode with an arbitrary parameter configuration, and the normal mode with a tuned parameter combination, we provide the average of the best objective values for 100 random permutations of variable indices. In order to examine possible effects of number of iterations, we conduct this experiment under two different number of iterations. 
%We then report the average values for each configuration, as well as the percentage difference between the objective values corresponding to the best and worst orderings. Our observation is that when the parameters for normal mode are not tuned, there is room for improvement with different variable orderings. In particular, the difference between the best and worst variable ordering decreases from about 24\% to 0.25\% with the tuning of parameters. For the parallel mode, however, this difference is already at an insignificant level, 0.03\%. So, we conclude that trying different variable orderings does not contribute much when normal mode parameters have already been tuned or when the parallel mode is being used. 
In the table, we also report the average percentage difference (Avg \% diff) of the objective values corresponding to the best and worst orderings where the differences are normalized with respect to the worst ordering.

The results suggest that while the impact of variable ordering is insignificant when the number of iterations is large, it affects the performance of DA when the number of iterations is small as the average normalized differences are significant. Additionally, we observe that when the parameters for normal mode are not tuned, there is a room for improvement with different variable orderings. In particular, with small number of iterations, the difference between the best and worst variable ordering decreases from about 42\% to 25\% with the tuning of parameters which is a significant improvement. Based on the table, in general, it is more reliable to work with larger iteration numbers as DA becomes insensitive to the input format.

\subsubsection{DA and the best exact solver comparison}
Based on the results provided above, we find out that GUROBI outperforms the other two state-of-the-art solvers, and DA in parallel mode has almost the same performance as the normal mode where parallel mode is robust in terms of variable ordering for larger iteration numbers. Thus, we choose to compare GUROBI and DA in parallel mode for further analysis. The results are presented in Figure \ref{fig:pureQUBO_da_vs_exact_solvers}.

For this comparison, first, we run  GUROBI with a time limit of 60 seconds in order to compare against DA's performance in the parallel mode, since the average run time of DA is obtained as 60 seconds. Figure \ref{subfig:pureQUBO_gap_dp_vs_gurobi_60} illustrates the results of this experiment. We observe that the performances of DA and GUROBI are almost the same except for small subset of the instances. We notice that while on the medium sized instances DA performs at least as good as GUROBI, on some larger instances GUROBI outperforms DA.
% We present our step-by-step comparison in Figure \ref{fig:pureQUBO_da_vs_exact_solvers}. In the figure, DA seems to do slightly better than GUROBI \nt{specially on some large instances}. In order to make the difference clear, we zoom into the last portion of Figure \ref{subfig:pureQUBO_gap_da_vs_gurobi} and display those parts in Figure \ref{subfig:pureQUBO_gap_da_vs_gurobi_zoomed}. We reach to the conclusion that DA is the best performing option here.  

After observing that there is only a slight difference in the gap values of DA and GUROBI, we test whether an increase in the time limit of GUROBI would help it to reach a better solution quality than DA. As a result of this last set of experiments for pure QUBO instances, in Figure \ref{subfig:pureQUBO_da_vs_gurobi_10min}, we plot the gap values of GUROBI obtained with a 10-minute time limit against those of DA (using 60 seconds on the average). From the figure, it seems like GUROBI in 10 minutes cannot improve the \% gap much and the results are close to DA. The results, also, imply that DA can reach to the almost same performance level as GUROBI in much shorter time.
% In Figure \ref{subfig:pureQUBO_gap_da_vs_gurobi_10min_zoomed}, we take a closer look into the parts in which they differ slightly, and observe that there is no clear winner in those parts. As such, we conclude that DA and GUROBI perform the same on the average in this case.


% \begin{figure}[ht]
%     \centering
% % 	\begin{subfigure}{0.49\textwidth}
% % 		\centering
% % 	    \includegraphics[scale=0.59]{figures/pureQUBO/qubo_gap_cgs_vs_da_45sec.png}
% % 		\caption{}
% % 		\label{subfig:pureQUBO_gap_da_vs_exact_solvers}
% % 	\end{subfigure}
% 	\begin{subfigure}{0.49\textwidth}
% 		\centering
%         \includegraphics[scale=0.62]{figures/pyFig/pureQUBO/qubo_gap_g_vs_da_45sec.pdf}
%         \caption{Full data set \nt{Analysis of full data set}}
%         \label{subfig:pureQUBO_gap_da_vs_gurobi}
% 	\end{subfigure}
% 	\begin{subfigure}{0.49\textwidth}
% 		\centering
%         \includegraphics[scale=0.62]{figures/pyFig/pureQUBO/qubo_gap_g_vs_da_45sec_zoom.pdf}
%         \caption{Subset of data set \nt{Magnification of the results of subset of data}}
%         \label{subfig:pureQUBO_gap_da_vs_gurobi_zoomed}
% 	\end{subfigure}
% 	\caption{Performance comparison of DA with GUROBI \nt{with 45-seconds time limit} for pure QUBO instances}
% 	\label{fig:pureQUBO_da_vs_exact_solvers}
% \end{figure}

\begin{figure}[ht]
    \centering
	\begin{subfigure}{0.49\textwidth}
		\centering
        \includegraphics[scale=0.62]{figures/newPureQUBO/Parallel_GUROBI_60s.pdf}
        \caption{60-second time limit for GUROBI}
        \label{subfig:pureQUBO_gap_dp_vs_gurobi_60}
	\end{subfigure}
	\begin{subfigure}{0.49\textwidth}
		\centering
        \includegraphics[scale=0.62]{figures/newPureQUBO/Parallel_60s_GUROBI_600s.pdf}
        \caption{10-minute time limit for GUROBI}
        \label{subfig:pureQUBO_da_vs_gurobi_10min}
	\end{subfigure}
	\caption{Performance comparison of DA modes with GUROBI for pure QUBO}
	\label{fig:pureQUBO_da_vs_exact_solvers}
\end{figure}



% \begin{figure}[H]
%     \centering
% 	\begin{subfigure}{0.49\textwidth}
% 		\centering
% 	    \includegraphics[scale=0.62]{figures/pyFig/pureQUBO/qubo_gap_g_vs_da.pdf}
% 		\caption{Full data set \nt{Analysis of full data set}}
% 		\label{subfig:pureQUBO_gap_da_vs_gurobi_10min}
% 	\end{subfigure}
% 	\begin{subfigure}{0.49\textwidth}
% 		\centering
%         \includegraphics[scale=0.62]{figures/pyFig/pureQUBO/qubo_gap_g_vs_da_zoom.pdf}
%         \caption{Subset of data \nt{Magnification of the results of subset of data}}
%         \label{subfig:pureQUBO_gap_da_vs_gurobi_10min_zoomed}
% 	\end{subfigure}
% 	\caption{Performance comparison of DA with GUROBI with 10-minute time limit for pure QUBO instances}
% 	\label{fig:pureQUBO_da_vs_gurobi}
% \end{figure}



Finally, we present a summary of our computational experiments on pure QUBO instances in Table \ref{tab:pureQUBO_summary} which reports average percentage gap (Avg \% gap) as well as average run time (Avg time). Based on the table, while the \% gap of GUROBI and DA are close and they outperform both CPLEX and SCIP, DA in normal mode can reach to a similar \% gap as DA in parallel mode and GUROBI in a very short amount of time on average. Therefore, in general, DA in normal mode produces the best results in QUBO benchmark problem instances. 

\input{tables/pureQUBO_summary}



\subsection{QAP Benchmarks}

Next, we test the performance of DA on a problem that is not originally defined as a QUBO problem but can easily be transformed into one. For this purpose, we choose the well-known Quadratic Assignment Problem, QAP, whose constraints are all equalities and all the decision variables are binaries. Different QUBO formulation of QAP are proposed in the literature. Authors in \cite{liu2019modeling} introduce a novel QUBO formulation for QAP which can overcome the limitation of DA i.e. restriction on the number of variables. The authors propose a local search based iterative algorithm which, in each iteration, aims to solve a QUBO formulation of QAP in various neighbourhoods. Although proposed formulation might yield better outcomes, considering several QUBO formulations is out of scope of this study. Mainly, in this work, we follow general steps for obtaining equivalent QUBO formulations of integer programming problems.


\subsubsection{Formulations}
We are given a set of $n$ facilities and a set of $n$ candidate locations. For each pair of locations $ \{k,\ell\} $, a distance parameter $d_{k\ell}$, and for each pair of facilities $ \{i,j\} $, a flow parameter $f_{ij}$ is defined. The goal is to assign all facilities to distinct locations by minimizing the sum of the distances multiplied by the corresponding flows. 

We define the decision variables as 
\begin{equation*}
    x_{ik} = 
    \begin{cases}
      1, & \text{if facility $i$ is assigned to location $k$} \\
      0, & \text{otherwise}
    \end{cases}
\end{equation*}

Then, using the parameters and variables defined above, an IP formulation for QAP can be written as follows:
\begin{subequations}
\begin{alignat}{2}
    \min \quad & \sum_{i=1}^{n} \sum_{j=1}^{n} \sum_{k=1}^{n} \sum_{\ell=1}^{n} f_{ij} \ d_{k\ell} \ x_{ik} \ x_{j\ell} &&  \label{eq:QAP_obj} \\[0.12cm]
    %
    \text{s.t.} & \sum_{i=1}^{n} x_{ik} = 1 && k \in \{1,\hdots,n\}  \label{eq:QAP_c1} \\
    & \sum_{k=1}^{n} x_{ik} = 1    && i \in \{1,\hdots,n\}  \label{eq:QAP_c2} \\
    %
    & x_{ik} \in \{0,1\}   && i \in \{1,\hdots,n\}, \ k \in \{1,\hdots,n\} \label{eq:QAP_c3}	
\end{alignat}
\end{subequations}
%explain the constraints here
The quadratic objective function \eqref{eq:QAP_obj} minimizes the total cost of the assignment. Constraints \eqref{eq:QAP_c1} ensure that each location is assigned exactly one facility, and \eqref{eq:QAP_c2} guarantee that each facility is assigned to a single location. Finally, constraints \eqref{eq:QAP_c3} enforce the decision variables to be binary.

Dualizing the equality (assignment) constraints, we obtain the following QUBO formulation of QAP:
\begin{subequations}
\begin{align}
\min\quad &{  \sum_{i=1}^{n} \sum_{j=1}^{n} \sum_{k=1}^{n} \sum_{\ell=1}^{n}  f_{ij} \ d_{k\ell} \ x_{ik} \ x_{j\ell} } + \penaltyCoef \sum_{k=1}^{n}\left(\sum_{i=1}^{n} x_{ik} - 1 \right)^2 +  \penaltyCoef \sum_{i=1}^{n}\left(\sum_{k=1}^{n} x_{ik} - 1 \right)^2  \label{eq:QAP_qubo_obj}\\[0.25cm]
%
\text{s.t.} \quad & x_{ik} \in \{0,1\} \qquad  i \in \{1,...,n\}, \ k \in \{1,...,n\} \label{eq:QAP_qubo_c}
\end{align}
\end{subequations}

\noindent where $\penaltyCoef > 0$ is the penalty coefficient. We note that, for a sufficiently large value of $\penaltyCoef$, the QUBO formulation for QAP provided in \eqref{eq:QAP_qubo_obj}--\eqref{eq:QAP_qubo_c} is exact; i.e., it produces provably optimal solutions for the original problem.




\subsubsection{Experimental results}

% We collect 136 QAP instances from the well-known library named QAPLIB\footnote{
% \href{http://qplib.zib.de}{http://qplib.zib.de}
% } \cite{furini2018qplib}. The instances have 144 to 10,000 variables. After filtering the instances that are eligible for DA, we are left with a total of 87 instances. Out of those, DA could only solve 12 of them, which constitute 15\% of the eligible instances, and encountered overflow errors for the remaining 85\%. In what follows, we present the experimental results obtained on this set of 12 instances, which have 256 or 1024 variables.


We collect 136 QAP instances from the well-known library named QAPLIB\footnote{
\href{http://qplib.zib.de}{http://qplib.zib.de}
} \cite{furini2018qplib}. The instances have 100 to 10,000 variables. After filtering the instances that are eligible for DA, we are left with a total of 123 instances. We solve those instances with DA in different modes and exact solvers when they are considered as both IP and QUBO solvers. Since DA experiments terminate in less than 2 minutes, we give 2-minute time limit to exact solvers in order to have a fair comparison. 

Table \ref{tab:QAP_feasibility} reports the percentage of the instances that solvers can find feasible solutions within the time limit (\% feasibility) as well as the average percentage gap (Avg \% gap) of the solvers on the instances for which DA fails to find any feasible solutions. From first row of the table, it can be observed that exact solvers as IP solvers are able to find feasible solutions to all QAP instances within two minutes. However, they fail to find any feasible solutions for a subset of instances as QUBO solvers. Among QUBO solvers, DA in normal and parallel modes outperform the others in terms of \% feasibility. Furthermore, second row of the table illustrates that although exact IP solvers can find feasible solutions for all of the instances, their average percentage gaps are too high in the instances for which normal and parallel modes of DA fail to find any feasible solutions. This implies that those instances are too hard so that the solvers struggle to come up with high quality solutions.

In order to have a better insight on the \% feasibility of DA, we choose a subset of instances that DA performs poorly on them and we scale the coefficients of the weight matrix down. We observe that with the new scaling \% feasibility of DA on the chosen instances increases from about 34\% to 75\% which implies the sensitivity of DA to the magnitude of the input coefficients. In what follows, we present the experimental results obtained on the original instances. Each figure, in this section, contains a list of common instances eligible for a particular comparison in which the instances are sorted based on the number of locations in them.

\input{tables/QAP_feasibilityTable}

We start with comparing the modes of DA, and exact solvers GUROBI, CPLEX, and SCIP to each other both as IP solvers and QUBO solvers. We evaluate the performance of the modes of DA based on the normalized difference of the upper bound values with respect to the normal mode of DA, which we define as $${100 \cdot (\text{UB}_\text{parallel}-\text{UB}_\text{normal})}/{|\text{UB}_\text{normal}|.}$$

Figure \ref{subfig:QAP_da_vs_da} illustrates the performance comparison of modes of DA on QAP instances. We observe that DA in parallel mode outperforms normal mode specially on small and medium sized instances. In what follows, we take the performance of GUROBI as an IP solver within 10-minute time limit as our reference performance and we report the normalized difference of the upper bound values with respect to it.

Next, in Figure \ref{fig:QAP_exact_comp} we compare solvers to each other. Figure \ref{subfig:QAP_IPsolvers_10min} shows the performance comparison of the exact solvers as IP solvers within 10-minute time limit. From the figure, it can be inferred that GUROBI performs better than CPLEX and SCIP in almost all of the instance, and SCIP performs poorly specially for large instances. In order to compare performance of the solvers as QUBO solvers we exclude SCIP. Since, based on Table \ref{tab:QAP_feasibility} it can barely find feasible solutions for the instances. Figure \ref{subfig:QAP_QUBOsolvers_10min} demonstrates the performance of GUROBI and CPLEX as QUBO solvers within 10-minute time limit. The figure shows that GUROBI outperforms CPLEX in general. Additionally, GUROBI as a QUBO solver provides higher quality solutions than GUROBI as an IP solver for a subset of instances when we compare it to our reference performance.


% \begin{figure}[ht]
%     \centering
% 	\begin{subfigure}{0.49\textwidth}
% 		\centering
% 	    \includegraphics[scale=0.62]{figures/pyFig/QAP/qap_normdiff_da_vs_da.pdf}
% 		\caption{}
% 		\label{subfig:QAP_da_vs_da}
% 	\end{subfigure}
% 	\begin{subfigure}{0.49\textwidth}
% 		\centering
%         \includegraphics[scale=0.62]{figures/pyFig/QAP/qap_gap_cg_10min.pdf}
%         \caption{}
%         \label{subfig:QAP_exact_solvers}
% 	\end{subfigure}
% 	\caption{Performance comparison of (a) DA modes, and (b) exact solvers for QAP}
% 	\label{fig:QAP_da_comp_exact_comp}
% \end{figure}

\begin{figure}[ht]
    \centering
	\includegraphics[scale=0.72]{figures/newQAP/QAP_DA2_Comp_normal.pdf}
	\caption{Performance comparison of DA modes with respect to DA normal}
	\label{subfig:QAP_da_vs_da}
\end{figure}


\begin{figure}[ht]
    \centering
	\begin{subfigure}{0.49\textwidth}
		\centering
	    \includegraphics[scale=0.62]{figures/newQAP/QAP_NormDiff_Solvers_600.pdf}
		\caption{10-minute time limit}
		\label{subfig:QAP_IPsolvers_10min}
	\end{subfigure}
	\begin{subfigure}{0.49\textwidth}
		\centering
        \includegraphics[scale=0.62]{figures/newQAP/QAP_NormDiff_solvers_QUBO_600.pdf}
        \caption{10-minute time limit}
        \label{subfig:QAP_QUBOsolvers_10min}
	\end{subfigure}
	\caption{Performance comparison of (a) IP solvers, and (b) QUBO solvers for QAP}
	\label{fig:QAP_exact_comp}
\end{figure}


%We observe from Figure \ref{subfig:QAP_da_vs_da} that\nt{, regardless of the size of the instances,} the \nt{normal} mode of DA clearly yields superior results compared to the \nt{parallel} mode. On the other hand, \nt{SCIP is outperformed by CPLEX and GUROBI according to the test results with a time limit of 10 minutes. By having a closer look to the figure, we can see that GUROBI performs slightly better than CPLEX on the test instances.}
%CPLEX and GUROBI perform almost the same according to the test results with a time limit of 10 minutes. In the following analysis, we only include the results of GUROBI as an exact solver. 

Next, we compare the performances of DA and GUROBI using the two plots in Figure \ref{fig:QAP_da_vs gurobi} where the plots demonstrate the superior performance of GUROBI both as an IP and a QUBO solver. Figure \ref{subfig:QAP_gap_da_vs_gurobi_IP} indicates that GUROBI as an IP solver within 2-minute time limit performs better than both modes of DA in general. Also, in this experiment, as we compare the performance of GUROBI to our reference performance, the figure implies that GUROBI cannot improve the quality of the solutions that much as the normalized difference of 2-minute results are almost zero. Figure \ref{subfig:QAP_gap_da_vs_gurobi_QUBO} confirms that GUROBI as a QUBO solver performs better than DA in normal mode when 1-minute time limit is given.

%indicates that the parallel mode of DA yields the best solutions. \nt{Figure \ref{subfig:QAP_gap_da_vs_gurobi_45sec} indicates that the normal mode of DA is outperformed by GUROBI and DA in parallel mode. From the figure, it is observed that DA in parallel mode yields better solution than GUROBI in one instance.} When we increase the time limit of GUROBI to 10 minutes, however, GUROBI does just as good as the parallel mode of DA.  

% \begin{figure}[ht]
%     \centering
% 	\begin{subfigure}{0.49\textwidth}
% 		\centering
% 	    \includegraphics[scale=0.62]{figures/pyFig/QAP/qap_gap_da_vs_da_vs_g_45sec.pdf}
% 		\caption{45-sec time limit for GUROBI}
% 		\label{subfig:QAP_gap_da_vs_gurobi_45sec}
% 	\end{subfigure}
% 	\begin{subfigure}{0.49\textwidth}
% 		\centering
%         \includegraphics[scale=0.62]{figures/pyFig/QAP/qap_gap_da_vs_g.pdf}
%         \caption{10-min time limit for GUROBI}
%         \label{subfig:QAP_gap_da_vs_gurobi_10min}
% 	\end{subfigure}
% 	\caption{Performance comparison of GUROBI and DA modes for QAP}
% 	\label{fig:QAP_da_vs gurobi}
% \end{figure}


\begin{figure}[ht]
    \centering
	\begin{subfigure}{0.49\textwidth}
		\centering
	    \includegraphics[scale=0.62]{figures/newQAP/QAP_NormDiff_Gurobi_120_DAs.pdf}
		\caption{2-minute time limit}
		\label{subfig:QAP_gap_da_vs_gurobi_IP}
	\end{subfigure}
	\begin{subfigure}{0.49\textwidth}
		\centering
        \includegraphics[scale=0.62]{figures/newQAP/QAP_NormDiff_DA_Normal_GUROBI_QUBO_60.pdf}
        \caption{1-minute time limit}
        \label{subfig:QAP_gap_da_vs_gurobi_QUBO}
	\end{subfigure}
	\caption{Performance comparison of DA and GUROBI (a) as an IP solver and (b) as a QUBO solver}
	\label{fig:QAP_da_vs gurobi}
\end{figure}




We conclude our experimental analysis for QAP with a summary of our computational findings, given in Table \ref{tab:QAP_summary}. It contains the average values from GUROBI both as an IP and QUBO solver with a 2-minute time limit, and from both modes of DA. The table reports average normalized difference with respect to our reference performance (Avg norm diff) and average run times (Avg time). In terms of solution quality, GUROBI as an IP solvers is the closest one to the reference performance and GUROBI as a QUBO solver is the second closest one. While GUROBI illustrates superior performance as an IP solver, from the table it is inferred that, given an extra amount of time, it improves the quality of the solutions only by 1.11\%. Finally, in terms of run times, DA in normal mode provides feasible solutions in significantly smaller amount of time than GUROBI and DA in parallel mode. By comparing the results presented in Figure \ref{subfig:QAP_da_vs_da} and Table \ref{tab:QAP_summary} for modes of DA, we conclude that parallel mode achieves better outcomes than the normal one.

%In terms of solution quality, the parallel mode DA is the best on the average, and GUROBI (as an IP solver) is the second best with a slight difference. In terms of run times, GUROBI (as an IP solver) does a bit better than both modes of DA, while solving the QUBO formulation of QAP with GUROBI yields inferior solutions compared to the ones of DA in parallel mode. 

\input{tables/QAP_summary}



==> TODO.tex <==



For each problem, add a sentence mentioning the \% gap performance, and say that if the LBs are reliable, then these are the results.

For SelCol, move the "\% solver gap row" to the end, and add \% feas values for IP results as well  (OK)
And change the table comments accordingly

==> tables/solvers_info.tex <==
\begin{table}[H]
	\centering
	\caption{Brief information about some solvers capable of solving QUBO problems}
	\label{tab:QUBO_solvers_info}
	\small
	\begin{tabular}{p{1.9cm}p{13.2cm}}
		\toprule
		\multicolumn{1}{l}{\bf Solver} & \multicolumn{1}{l}{\bf Problem Type} \\
		\midrule
        { CPLEX} &  MIQP, MIQCP  \\[0.2cm]
        %\midrule
        { GUROBI} & MIQP, MIQCP \\[0.2cm]
        %\mudrule
        { SCIP} & MIQP, MIQCP \\[0.2cm]
        { MIOSQP} & MIQP %(based on OSQP solver) %\citep{osqp,stellato2018embedded} 
        \\[0.2cm]
        { MOSEK} &  MIQP, MIQCP (except quadratic objective/constraints $+$ conic constraints) \\[0.2cm]
        { GLOMIQO} & MIQP, MIQCP % available through GAMS
        \\[0.2cm]
        { BARON} &  MIQP, MIQCP % available under the AIMMS, AMPL, and GAMS modeling languages  
        \\[0.2cm]
		\bottomrule
	\end{tabular}%
\end{table}%

==> unused/QuadCycleCover_withMeijerComp.tex <==
\section{Quadratic Cycle Cover Problem}

After making an initial assessment of DA's performance, we now explore {\cred a new application of DA -- REPHRASE!}. Cycle Cover Problem (CCP) is a well-known combinatorial optimization problem which is a relaxation of Travelling Salesman Problem (TSP) \cite{khachay2016}. 
Given a graph $G=(V,A)$ with a vertex set $V$ and an arc set $A$, a {\it cycle cover} of $G$ is a set of cycles in the graph which visits all of its vertices. A disjoint cycle cover is a cycle cover where each vertex is visited by exactly one cycle. Using these terminology, CCP is a problem of finding a minimum weight disjoint cycle cover in the given graph. In this study we consider Quadratic Cycle Cover Problem (QCCP) which aims to find a disjoint cycle cover on graph $G$ so that the summation of the correlation costs between adjacent arcs is minimized.


\subsection{Formulations}

Given a directed graph $G=(V,A)$ with a vertex set $V = \{1,...,n\}$ and an arc set $A \subseteq V \times V$, as well as a cost matrix $Q \in \R^{|A| \times |A|}$, a QCCP instance can be identified by the pair $(G,Q)$. 
QCCP can be formulated as an integer programming (IP) problem which includes only binary variables and equality constraints. 
In this problem,the entries of matrix $Q$ are nonzero if the corresponding arcs are consecutive. 
In other words, if the ending vertex of arc $a_1 \in A$ and beginning vertex of arc $a_2 \in A$ are the same, then, $Q_{{a_1}{a_2}}$ can be nonzero.


%In order to model QCCP, 
Let $\delta^{+}(i)$ ($\delta_{-}(i)$) denote the set of all outgoing (incoming) arcs of vertex $i \in V$. 
We define binary decision variables $x_{a}$'s for $a$ in $A$ in order to follow the assignment of each arc to a cycle.
\begin{equation*}
    x_a = 
    \begin{cases}
        1, & \text{if arc $a$ is assigned to a cycle} \\
      0, & \text{otherwise}
    \end{cases}
\end{equation*}
Then, an IP formulation for QCCP can be written as follows:
\begin{subequations}
\begin{alignat}{2}
	\min\quad &{\sum_{a_1 \in A}\sum_{\substack{a_2: a_2 \in A,\\ \phantom{aaa}a_1 \neq a_2}} q_{{a_1}{a_2}} \ x_{a_1} \ x_{a_2}} \label{eq:QCCP_IP_obj}\\
	\text{s.t.} \quad &{ \sum_{a \in \delta^{+}(i)} x_{a} = 1} \qquad && { i \in V } \label{eq:QCCP_IP_c1} \\[0.1cm]
	%
	&{ \sum_{a \in \delta^{-}(i)} x_{a} = 1} && {i \in V} \label{eq:QCCP_IP_c2}\\[0.1cm]
	%
	& x_{a} \in \{0,1\} && {a \in A} \label{eq:QCCP_IP_c3}
\end{alignat}
\label{m:qccp}
\end{subequations}
The quadratic objective function \eqref{eq:QCCP_IP_obj} minimizes the total sum of the interaction cost between adjacent arcs. Constraints \eqref{eq:QCCP_IP_c1} and \eqref{eq:QCCP_IP_c2} ensure that each vertex must be visited by exactly one cycle. Constraints \eqref{eq:QCCP_IP_c3} restricts decision variables to be binary.

Similar to QAP, we can dualize the equality constraints and obtain the QUBO formulation for QCCP as follows:
\begin{subequations}
\begin{align}
\min\quad &{ \sum_{a_1 \in A} \sum_{\substack{a_2: a_2 \in A,\\ \phantom{aaa}a_1 \neq a_2}} q_{{a_1}{a_2}} \ x_{a_1} \ x_{a_2} } + \penaltyCoef \sum_{i \in V}\left(\sum_{a \in \delta^{+}(i)} x_{a} - 1 \right)^2 +  \penaltyCoef \sum_{i \in V}\left(\sum_{ a \in \delta^{-}(i)} x_{a} - 1 \right)^2  \label{eq:QCCP_qubo_obj}\\[0.25cm]
%
\text{s.t.} \quad & x_{a} \in \{0,1\} \qquad  a \in A \label{eq:QCCP_qubo_c}
\end{align}
\label{m:qccp_qubo}
\end{subequations}
\noindent where $\penaltyCoef > 0$ is the penalty coefficient. We note that, for a sufficiently large value of $\penaltyCoef$, the QUBO formulation \eqref{m:qccp_qubo} produces provably optimal solutions for the original IP model \eqref{m:qccp}.


\subsection{Experimental results}

HOW WE GENERATED THE INSTANCES, INTRODUCE WHAT YOU MEAN BY 'MAIN' SET OF INSTANCES AND MEIJER

THAT IT IS NOT EASY TO GUARANTEE THE FEASIBILITY OF A PROBLEM INSTANCE, WHAT WE USED TO PARTIALLY ALLEVIATE THIS DIFFICULTY, AND THAT ALL OF OUR PROBLEM INSTANCES TURNED OUT TO BE FEASIBLE

INFO ON THE MOTIVATION FOR MEIJER INSTANCES

% Table generated by Excel2LaTeX from sheet 'Instance_info'
\begin{table}[htbp]
  \centering
  \caption{QCCP instance information.}
   \def\arraystretch{1.15}%  1 is the default, change whatever you need
  \scalebox{1}{
    \begin{tabular}{ccccc}
    \toprule
      & \parbox[t]{1.5cm}{\centering \# inst} & \parbox[t]{1.5cm}{\centering \# nodes} & \parbox[t]{1.5cm}{\centering Density} & \parbox[t]{1.5cm}{\centering \# vars} \\
    \midrule
    Main  & 80    & [25, 175] & \{0.25, 0.50, 0.75\} & [127, 7963] \\
    Meijer type & 15    & [20, 80] & \{0.30, 0.50\} & [144, 1887] \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:qcc_inst_info}%
\end{table}%


In the figures that follow, we present the results from our 60-second experiments, which involve our main set of instances as well as those {\cred for Meijer comparison}. 
The points on the $x$-axes of figures represent individual instances arranged in ascending order with respect to the number of variables they have.
We note that increasing the time limit to 120 seconds does not much change the general picture, and hence results of 60-second experiments suffice to make a fair comparison.

\os{EXPLAIN WHY WE USE NORMALIZED DIFFERENCE IN OUR COMPARATIVE ANALYSIS AND WHY WE EXCLUDE LOWER BOUNDS}

We begin with comparing the performance of GUROBI and CPLEX in solving the \os{IP formulation ???} under 60-second time limit.
We do not include SCIP in this comparison, because it failed to deliver any lower or upper bound, even when the time limit is increased to 120 seconds.
Figure \ref{fig:qcc_cplex_vs_gurobi_normUBdiff} shows the normalized difference of the upper bounds (``Norm UB diff"), where the upper bounds (UBs) from GUROBI's 10-minute experiments are taken as a reference. 
Namely, it is calculated as 
\begin{align*}
\text{Norm UB diff} \ = \ \frac{\text{UB} - \text{UB}_{\text{GUROBI (10-min)}}}{\text{UB}_{\text{GUROBI (10-min)}}}.
\end{align*}
%$$ \text{Norm UB diff} \ = \ \frac{\text{UB} - \text{UB}_{\text{GUROBI (10-min)}}}{\text{UB}_{\text{GUROBI (10-min)}}} $$. 

We see from Figure \ref{subfig:qcc_cplex_vs_gurobi_normUBdiff_main} that GUROBI mostly outperforms CPLEX in our main set of instances, by providing significantly lower UB values especially for moderate-size instances.
This observation is valid for {\cred Meijer type instances} as well.
In particular, GUROBI does at least as well as CPLEX in nearly 73\% and 94\% of the main and {\cred Meijer type instances}, respectively.
Thus, we use GUROBI in the rest of our analysis to compare DA's performance to.

\begin{figure}[ht]
    \centering
	\begin{subfigure}{0.49\textwidth}
		\centering
	    \includegraphics[scale=0.62]{figures/QCC/fig_QCC_normUBDiff_CPLEX_vs_GUROBI_60sec.pdf}
		\caption{\os{60-second time limit}}
		\label{subfig:qcc_cplex_vs_gurobi_normUBdiff_main}
	\end{subfigure}
	\begin{subfigure}{0.49\textwidth}
		\centering
        \includegraphics[scale=0.62]{figures/QCC/fig_QCC_normUBDiff_CPLEX_vs_GUROBI_60sec_forMeijerComparison.pdf}
        \caption{\os{60-second time limit Meijer}}
        \label{subfig:qcc_cplex_vs_gurobi_normUBdiff_Meijer}
	\end{subfigure}
	\caption{Performance comparison of CPLEX and GUROBI for QCC using norm UB diff}
	\label{fig:qcc_cplex_vs_gurobi_normUBdiff}
\end{figure}


Next, we compare the performances of DA and GUROBI.
Figure \ref{fig:qcc_da_vs_gurobi_normUBdiff} shows the normalized UB differences for GUROBI and both modes of DA.
We observe from Figure \ref{subfig:qcc_da_vs_gurobi_normUBdiff_main} that for relatively small instances GUROBI yields better UBs than DA.
On the other hand, for larger instances, i.e., when we look at the data points towards the right of the $x$-axis, both normal and parallel modes of DA yield significantly better UB values, with the parallel mode being the best among all.
Such instances comprise about 29\% of our main set of instances and have 4500 or more variables.
It is also noteworthy that the gap between the data points corresponding to GUROBI and the parallel mode of DA is greater for larger instances, and that DA shows a robust performance with increasing instance sizes.
For the {\cred Meijer type instances}, we see from Figure \ref{subfig:qcc_da_vs_gurobi_normUBdiff_Meijer} that GUROBI is the outperformer throughout all the instances, which can well be attributed to the fact that this set is comprised of small instances. 
Hence, we conclude that DA is particularly successful in quickly yielding good-quality solutions for large instances.

\begin{figure}[ht]
    \centering
	\begin{subfigure}{0.49\textwidth}
		\centering
	    \includegraphics[scale=0.62]{figures/QCC/fig_QCC_normUBDiff_DA2_vs_GUROBI_allDAmodes_60sec.pdf}
		\caption{\os{60-second time limit}}
		\label{subfig:qcc_da_vs_gurobi_normUBdiff_main}
	\end{subfigure}
	\begin{subfigure}{0.49\textwidth}
		\centering
        \includegraphics[scale=0.62]{figures/QCC/fig_QCC_normUBDiff_DA2_vs_GUROBI_allDAmodes_60sec_forMeijerComparison.pdf}
        \caption{\os{60-second time limit Meijer}}
        \label{subfig:qcc_da_vs_gurobi_normUBdiff_Meijer}
	\end{subfigure}
	\caption{Performance comparison of DA and GUROBI for QCC using norm UB diff}
	\label{fig:qcc_da_vs_gurobi_normUBdiff}
\end{figure}


In our last set of results, we investigate the effect of the penalty coefficient values on DA’s performance. 
Figure \ref{fig:qcc_pentrials} shows the average of the best objective values found by DA using six different penalty coefficient values on our main set of problem instances.
We first see that the parallel mode of DA delivers significantly better results than the normal mode on the average.
In addition, setting $\penaltyCoef = 1000$ gives the least overall average values for parallel mode, and the performance keeps deteriorating for larger values of the penalty coefficient $\penaltyCoef$.
As the parallel mode yields better results in general, we took its minimum point as a reference and used $\penaltyCoef = 1000$ when running the QUBO models for QCCP.
%The penalty coefficients that we test do not necessarily guarantee that infeasible solutions are always associated with larger objective values than feasible solutions (since we are minimizing).

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.62]{figures/QCC/fig_QCC_penTrials.pdf}
	\caption{Penalty coefficient trials for QCC}
	\label{fig:qcc_pentrials}
\end{figure}


In the remainder of this section, we provide tabular summaries of overall performances.
We first present the average performance of solving the QUBO formulation with DA in comparison to solving the IP formulations with GUROBI, CPLEX and SCIP on our main set of instances under different time limits, reported in Table \ref{tab:qcc_summary_main}.
The table contains three blocks of columns reserved for different time limits, and another column dedicated to the normal mode of DA only, because its execution times do not exceed half a second even when the number of iterations is increased greatly. 
The blocks contain the results of solving the QUBO formulations with DA and/or solving the IP formulations with GUROBI, CPLEX and SCIP.
For each option (column), we report the averages of UBs (``UB"), normalized difference of UBs (``UB"), and solution times (``Time (sec)").
We note that the normalized differences are calculated using the UB values from 10-minute experiments with GUROBI, as it yielded the most promising values.
Furthermore, SCIP is excluded from 60-second and 120-second blocks, because it failed to yield any valid LB or UB within these time limits, as mentioned before.

Under 60-second and 120-second time limits, parallel mode of DA gives the best average UB values, and the difference is considerably large in the 60-second case.
As for the normal mode, its average UB is better than those obtained from CPLEX and SCIP under 10-minute limit, and its execution time is only 0.39 second. 
%So, we can say that in cases where good-quality solutions are needed in a matter of a second or even less, normal mode of DA is best option.
In terms of the average normalized UB differences, GUROBI averages are the best under all three time limits.
Combining these aggregated results with those over the individual instances discussed above, we can say that DA is particularly successful in yielding good-quality solutions for relatively large instances, and if such solutions are needed within a second, normal mode of DA is the most promising option.
We note that all the solutions that DA yield are feasible, and hence is not explicitly reported in the table.


% Table generated by Excel2LaTeX from sheet 'SUMMARY (2)'
\begin{table}[htbp]
  \centering
  \caption{DA AND BIP SOLVER RESULTS FOR THE MAIN 80 INSTANCES}
  \def\arraystretch{1.15}%  1 is the default, change whatever you need
  \scalebox{0.9}{
    \begin{tabular}{c S[table-format=4.2] S[table-format=4.2] S[table-format=4.2] S[table-format=4.2] S[table-format=4.2] S[table-format=4.2] S[table-format=4.2] S[table-format=4.2] S[table-format=4.2] S[table-format=4.2]}
    \toprule
      &       & \multicolumn{3}{c}{60-sec limit} & \multicolumn{3}{c}{120-sec limit} & \multicolumn{3}{c}{10-min limit} \\
      \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
      & \parbox[t]{1.1cm}{\centering DA (n)} & \parbox[t]{1.1cm}{\centering DA (p)} & \parbox[t]{1.1cm}{\centering GUROBI} & \parbox[t]{1.1cm}{\centering CPLEX}  & \parbox[t]{1.1cm}{\centering DA (p)}  & \parbox[t]{1.1cm}{\centering GUROBI} & \parbox[t]{1.1cm}{\centering CPLEX} & \parbox[t]{1.1cm}{\centering GUROBI} & \parbox[t]{1.1cm}{\centering CPLEX} & \parbox[t]{1.1cm}{\centering SCIP} \\
    \midrule
    UB & 2803.73 & 2059.53 & 2573.51 & 3311.90 & 2057.60 & 2152.60 & 3222.05 & 1105.68 & 2812.90 & 3522.44 \\
    Norm UB diff & 172.12 & 129.54 & 90.02 & 173.28 & 128.23 & 63.80 & 161.59 & 0.00  & 112.58 & 199.34 \\
    Time (sec) & 0.39  & 61.65 & 56.28 & 57.40 & 103.77 & 112.01 & 114.35 & 541.02 & 563.73 & 567.08 \\
    %\% feasible & 1.00  & 1.00  &       &       & 1.00  &       &       &       &       &  \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:qcc_summary_main}%
\end{table}%


We now evaluate the overall performances of GUROBI, CPLEX and SCIP in solving the QUBO formulations from our main set of problem instances, and report the associated results in Table \ref{tab:qcc_summary_qubo_main}.
In this case, since we are solving QUBO models, we include the percentage of found solutions that are feasible (``\% feas") in addition to the three measures used in Table \ref{tab:qcc_summary_main}.
We see from the last row of the table that SCIP fails to deliver any feasible solution within one minute, and in two minutes, it only achieves feasibility in about 6\% of the instances.
Even though GUROBI and CPLEX does significantly better relative to SCIP, their QUBO-solving performance is still not satisfactory; the feasibility percentage cannot go above 68\% in the best case. 


% Table generated by Excel2LaTeX from sheet 'SUMMARY (2)'
\begin{table}[htbp]
  \centering
  \caption{QUBO SOLVER RESULTS FOR THE MAIN 80 INSTANCES}
  \def\arraystretch{1.15}%  1 is the default, change whatever you need
  \scalebox{0.94}{
    \begin{tabular}{c S[table-format=6.2] S[table-format=4.2] S[table-format=6.2] S[table-format=5.2] S[table-format=4.2] S[table-format=6.2]}
    \toprule
      & \multicolumn{3}{c}{60-sec limit} & \multicolumn{3}{c}{120-sec limit} \\
      \cmidrule(lr){2-4}\cmidrule(lr){5-7}
      & \parbox[t]{1.4cm}{\centering GUROBI} & \parbox[t]{1.4cm}{\centering CPLEX} & \parbox[t]{1.4cm}{\centering SCIP} & \parbox[t]{1.4cm}{\centering GUROBI} & \parbox[t]{1.4cm}{\centering CPLEX} & \parbox[t]{1.4cm}{\centering SCIP} \\
    \midrule
    UB & 91802.80 & 6143.74 & 158424.02 & 77820.23 & 5967.74 & 157672.86 \\
    Norm UB diff & 5701.38 & 453.28 & 15236.51 & 4106.86 & 416.52 & 14924.22 \\
    Time (sec) & 60.82 & 103.27 & 60.35 & 120.17 & 138.58 & 121.14 \\
    \% feas & 55.00  & 30.00  & 0.00  & 67.50  & 32.50  & 6.25 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:qcc_summary_qubo_main}%
\end{table}%


In the last two tables that follow, we present the same set of overall results for {\cred Meijer-type instances}.
Our observation from Tables \ref{tab:qcc_summary_Meijer} and \ref{tab:qcc_summary_qubo_Meijer} is that GUROBI delivers the best results in this set of relatively small instances, even when it solved the QUBO formulation.
We see that the performance of GUROBI in solving the QUBO formulations is better than either mode of DA.
Yet, normal mode of DA is still quite successful in delivering reasonably good solutions in 0.39 second on the average, in which other solvers fail to even complete the presolve phase typically.


COMPARE THE RESULTS WITH THOSE IN THE MEIJER PAPER!!!!


% Table generated by Excel2LaTeX from sheet 'SUMMARY (2)'
\begin{table}[htbp]
  \centering
  \caption{DA AND BIP SOLVER RESULTS FOR THE MEIJER TYPE INSTANCES}
  \def\arraystretch{1.15}%  1 is the default, change whatever you need
  \scalebox{0.82}{
    \begin{tabular}{c S[table-format=4.2] S[table-format=4.2] S[table-format=3.2] S[table-format=3.2] S[table-format=4.2] S[table-format=4.2] S[table-format=3.2] S[table-format=3.2] S[table-format=4.2] S[table-format=3.2] S[table-format=3.2] S[table-format=4.2]}
    \toprule
      &  & \multicolumn{4}{c}{60-sec limit} & \multicolumn{4}{c}{120-sec limit}   & \multicolumn{3}{c}{10-min limit} \\
      \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-13}
      & \parbox[t]{1cm}{\centering DA (n)} & \parbox[t]{1cm}{\centering DA (p)} & \parbox[t]{1cm}{\centering GUROBI} & \parbox[t]{1cm}{\centering CPLEX}  & \parbox[t]{1cm}{\centering SCIP}  & \parbox[t]{1cm}{\centering DA (p)}  & \parbox[t]{1cm}{\centering GUROBI} & \parbox[t]{1cm}{\centering CPLEX} & \parbox[t]{1cm}{\centering SCIP} & \parbox[t]{1cm}{\centering GUROBI} & \parbox[t]{1cm}{\centering CPLEX} & \parbox[t]{1cm}{\centering SCIP} \\
    \midrule
    UB & 1178.67 & 1088.60 & 549.07 & 775.80 & 1533.40 & 1088.60 & 514.53 & 656.87 & 1406.80 & 448.00 & 531.47 & 1191.33 \\
    Norm UB diff & 189.14 & 182.37 & 22.66 & 71.65 & 250.03 & 182.37 & 15.21 & 49.33 & 210.70 & 0.00  & 26.91 & 153.78 \\
    Time (sec) & 0.39  & 65.27 & 51.23 & 57.37 & 60.02 & 109.28 & 95.23 & 107.71 & 120.00 & 401.85 & 460.40 & 528.64 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:qcc_summary_Meijer}%
\end{table}%


% Table generated by Excel2LaTeX from sheet 'SUMMARY (2)'
\begin{table}[htbp]
  \centering
  \caption{QUBO SOLVER RESULTS FOR THE MEIJER TYPE INSTANCES}
  \def\arraystretch{1.15}%  1 is the default, change whatever you need
  \scalebox{0.94}{
    \begin{tabular}{c S[table-format=3.2] S[table-format=4.2] S[table-format=5.2] S[table-format=3.2] S[table-format=4.2] S[table-format=5.2]}
    \toprule
      & \multicolumn{3}{c}{60-sec limit} & \multicolumn{3}{c}{120-sec limit} \\
      \cmidrule(lr){2-4}\cmidrule(lr){5-7}
      & \parbox[t]{1.4cm}{\centering GUROBI} & \parbox[t]{1.4cm}{\centering CPLEX} & \parbox[t]{1.4cm}{\centering SCIP} & \parbox[t]{1.4cm}{\centering GUROBI} & \parbox[t]{1.4cm}{\centering CPLEX} & \parbox[t]{1.4cm}{\centering SCIP} \\
  \midrule
    UB & 569.93 & 1909.93 & 59097.68 & 548.60 & 1894.67 & 53204.88 \\
    Norm UB diff & 40.64 & 213.18 & 12565.42 & 34.68 & 207.75 & 11264.10 \\
    Time (sec) & 60.04 & 56.65 & 60.15 & 120.02 & 104.72 & 120.16 \\
    \% feas & 100.00  & 80.00  & 0.00  & 100.00  & 80.00  & 20.00 \\
    \bottomrule
    \end{tabular}%
    }
  \label{tab:qcc_summary_qubo_Meijer}%
\end{table}%





















\begin{comment}
\begin{figure}[ht]
    \centering
	\begin{subfigure}{0.49\textwidth}
		\centering
	    \includegraphics[scale=0.62]{figures/QCC/fig_QCC_normUBDiffDiff_CPLEX_vs_GUROBI_60sec.pdf}
		\caption{\os{60-second time limit}}
		\label{subfig:}
	\end{subfigure}
	\begin{subfigure}{0.49\textwidth}
		\centering
        \includegraphics[scale=0.62]{figures/QCC/fig_QCC_normUBDiffDiff_CPLEX_vs_GUROBI_60sec_forMeijerComparison.pdf}
        \caption{\os{60-second time limit Meijer}}
        \label{subfig:}
	\end{subfigure}
	\caption{Performance comparison of CPLEX and GUROBI for QCC using norm UB diff diff}
	\label{fig:qcc_cplex_vs_gurobi_normUBdiffdiff}
\end{figure}


\begin{figure}[ht]
    \centering
	\begin{subfigure}{0.49\textwidth}
		\centering
	    \includegraphics[scale=0.62]{figures/QCC/fig_QCC_normUBDiffDiff_DA2_vs_GUROBI_60sec.pdf}
		\caption{\os{60-second time limit}}
		\label{subfig:}
	\end{subfigure}
	\begin{subfigure}{0.49\textwidth}
		\centering
        \includegraphics[scale=0.62]{figures/QCC/fig_QCC_normUBDiffDiff_DA2_vs_GUROBI_60sec_forMeijerComparison.pdf}
        \caption{\os{60-second time limit Meijer}}
        \label{subfig:}
	\end{subfigure}
	\caption{Performance comparison of CPLEX and GUROBI for QCC using norm UB diff diff}
	\label{fig:qcc_da_vs_gurobi_normUBdiffdiff}
\end{figure}
\end{comment}

